DiscreteSLU: A Large Language Model with Self-Supervised Discrete Speech Units for Spoken Language Understanding

The integration of pre-trained text-based large language models (LLM) with speech input has enabled instruction-following capabilities for diverse speech tasks. This integration requires the use of a speech encoder, a speech adapter, and an LLM, trained on diverse tasks. We propose the use of discrete speech units (DSU), rather than continuous-valued speech encoder outputs, that are converted to the LLM token embedding space using the speech adapter. We generate DSU using a self-supervised speech encoder followed by k-means clustering. The proposed model shows robust performance on speech inputs from seen/unseen domains and instruction-following capability in spoken question answering. We also explore various types of DSU extracted from different layers of the self-supervised speech encoder, as well as Mel frequency Cepstral Coefficients (MFCC). Our findings suggest that the ASR task and datasets are not crucial in instruction-tuning for spoken question answering tasks.

==> tables/prompt_example.tex <==

\begin{table}[t]\centering
\caption{Prompt with SLUE-SQA5 data example}\label{tab:prompt_example}
\begin{tabular}{ll}
\toprule
Instruction: & What did Roland Bainton say about \\
 &   Luther's position on Jews? \\
Input: &20 32 44 21 295 185 ... 998 29 2 44 842  \\
Output: &entirely religious and in no respect racial \\ 
\bottomrule
\end{tabular}
\end{table}
